Tight Typings and Split Bounds

Multi types---aka non-idempotent intersection types---have been used to obtain quantitative bounds on higher-order programs, as pioneered by de Carvalho. Notably, they bound at the same time the number of evaluation steps and the size of the result. Recent results show that the number of steps can be taken as a reasonable time complexity measure. At the same time, however, these results suggest that multi types provide quite lax complexity bounds, because the size of the result can be exponentially bigger than the number of steps. Starting from this observation, we refine and generalise a technique introduced by Bernadet & Graham-Lengrand to provide exact bounds for the maximal strategy. Our typing judgements carry two counters, one measuring evaluation lengths and the other measuring result sizes. In order to emphasise the modularity of the approach, we provide exact bounds for four evaluation strategies, both in the lambda-calculus (head, leftmost-outermost, and maximal evaluation) and in the linear substitution calculus (linear head evaluation). Our work aims at both capturing the results in the literature and extending them with new outcomes. Concerning the literature, it unifies de Carvalho and Bernadet & Graham-Lengrand via a uniform technique and a complexity-based perspective. The two main novelties are exact split bounds for the leftmost strategy---the only known strategy that evaluates terms to full normal forms and provides a reasonable complexity measure---and the observation that the computing device hidden behind multi types is the notion of substitution at a distance, as implemented by the linear substitution calculus.

==> 2.1-memory-bis.tex <==
% !TEX root = main.tex
\subsection{Using Klop's memory operator}
\label{s:klop-calculus}

The syntax at work is that of the pure $\l$-calculus enriched with a memory
operator. The set of $\mem$-terms denoted by $\lterms_{\mem}$ is defined by means of the following grammar:  
\[ \begin{array}{lll}
   \tm, \tmtwo  & :: =  &  \var \mid  \l \var. \tm  \mid \tm \tmtwo  \mid  \tm\mm{\tmtwo} \\ 
   \end{array} \] 
The notion of \emph{free} variable is defined as expected, in particular,
$\fv{\tm\mm{\tmtwo}} :=
\fv{\tm} \cup \fv{\tmtwo}$. %$\bv{\tm\mm{\tmtwo}}:= \bv{\tm} \cup \bv{\tmtwo} $.
%% \delia{We write  $\numfv{\tm}{\var}$ to denote  the number
%% of \emph{occurrences} of $\var$ that are in $\fv{\tm}$.}
The constructor $\cdot \mm{\cdot}$ is called a  \emph{memory operator}.
We restrict the set $\lterms_\mem$ to the \emph{admissible} ones:
$\tm$ is  \emph{admissible}
if every subterm of the form $\l \var. \tmtwo$ in $\tm$
verifies $\var \in \fv{\tmtwo}$. From now on all the $\mem$-terms
are supposed to be admissible, without stating it explicitely.
\delia{For each variable $\var$, we write $\specialterms{\var}$
the sets of \emph{special} terms of the form $\tm\mm{\var}$ where $\var \notin \fv{\tm}$. }

%% \delia{Free variables can occur \emph{inside} (resp. \emph{outside}) memory operators.
%%   We write $\ifv{\tm}$ (resp. $\ofv{\tm}$) for the
%%   variables occuring \emph{only}
%%   inside (resp. outside) memory operators. 
%% For example $\ifv{\var\vartwo \mm{\var \varthree}} = \set{\varthree}$
%% and $\ofv{\var\vartwo \mm{\var \varthree}} = \set{\vartwo}$.
%% We write  $\numifv{\tm}{\var}$
%% to denote  the number of \emph{occurrences} 
%% of $\var$ that are in $\ifv{\tm}$. 
%% Thus for example
%% $\numifv{\vartwo\mm{\var}}{\var}=1$,
%% $\numifv{\vartwo\mm{\var}\vartwo\mm{\var}}{\var}=\numifv{\vartwo\mm{\var\var}}{\var}=2$
%% and $\numifv{\var\mm{\var\var}}{\var}=0$.}


%%Free variables inside memory operators of $\tm$ are called \emph{memory free variables},
%%they are  denoted by $\mfv{\tm}$ and defined as expected.  
%%
%% We restrict the set $\lterms_\mem$ by an \emph{admissibility}
%% predicate $\adm{\cdot}$ defined as follows:
%% \[ \infer{\adm{\var} }
%%          {\phantom{\adm{\var} }} \msep
%%          \infer{
%%         \adm{\tm \tmtwo}}
%%          {\adm{\tm} \msep \adm{\tmtwo}} \msep
%%    \infer{\adm{\tm \mm{\tmtwo}}}
%%          {\adm{\tm} \msep \adm{\tmtwo}} \msep
%%      \infer{\adm{\l \var. \tm} }{\adm{\tm}\msep \var \in \fv{\tm} \setminus \mfv{\tm}}  \msep     
%%     \infer{\adm{\l \var. \tm\mm{\var}} }{\adm{\tm}\msep \var \notin \fv{\tm}}           \]
%%     Remark in particular that every admissible abstraction $\l \var. \tm$
%%     verifies $\var \in \fv{\tm}$. Moreover, a variable inside a memory operator can
%%     only be bound once, \ie\ the  term $\l \var. \vartwo \mm{\var}\mm{\var}$ is
%%     not admissible but the term $\vartwo \mm{\var}\mm{\var}$ is admissible. 



\paragraph{Normal, neutral and abs predicates.} The notions of spine/skeleton neutral/normal 
forms and abs are  extended to 
$\mem$-terms as expected in \reffig{normalformsmemory}. 
An $\mem$-term $\tm$ is said to be
\emph{memory-normal}, written $\fullymemnorm{\tm}$,  if $\skenormmem{\tmthree}$
for every subterm
$\tmtwo \mm{\tmthree}$ of $\tm$.

\paragraph{Small-step semantics.} (\emph{Non-deterministic}) 
skeleton evaluation $\toperp$ for $\mem$-terms
is defined in \reffig{memory-discipline}. Remark that 
$\toperp$ evaluation does not erase any term since
every abstraction $\l \var. \tm$ verifies $\var \in \fv{\tm}$.
The \emph{deterministic} memory strategy, simply written  $\toperpp$, is defined in
\reffig{memory-deterministic}.  
Note that the  deterministic  strategy $\toperpp$ can be obtained as a particular case of
the evaluation relation $\toperp$. 
We use the notations
$\toperplus{k}, \toperpp^k$ and $\toperpet, \toperpp^*$ for the transitive and
reflexive-transitive closures as before.
Here is an example of evaluation: 
$(\l \var. \l  \vartwo. \vartwo\mm{\var})  \var' \vartwo'
\toperp  (\l \vartwo. \vartwo)\mm{\var'}  \vartwo' \toperp  \vartwo'\mm{\var'}$.
Remark that the term $\tm_0 = \vartwo'\mm{\var'} $ 
cannot be evaluated anymore,  \ie\ $ \skenormmem{\tm_0}$.
Another example is
$\tm_1=(\l \varthree. (\l \var. \tm \mm{\var}) (\varthree \varthree)) \tmtwo \toperp
(\l \varthree.  \tm \mm{\varthree \varthree})  \tmtwo \toperp
\tm \mm{\tmtwo \tmtwo}=\tm_2$, \delia{remark that the deterministic step $\tm_1 \toperpp (\l \varthree.  \tm \mm{\varthree \varthree})  \tmtwo$
does not hold, but the same normal form $\tm_2$ can be obtained by the following
deterministic sequence $\tm_1 \toperpp  (\l \var. \tm \mm{\var}) ( \tmtwo  \tmtwo) \toperpp \tm\mm{\tmtwo  \tmtwo} $}. 


\paragraph{Sizes.} The notion of  \emph{size} 
is extended to  $\mem$-terms as expected:
\[ \begin{array}{llllll} 
   \multicolumn{3}{c}{\textsc{Memory Skeleton size}}\\
   \syssize\systemem \var & := & 0 & 
   \syssize\systemem { \tm \tmtwo} & :=& \syssize\systemem \tm + \syssize\systemem \tmtwo+ 1\\
   \syssize\systemem {\l \var. \tm} & :=& \syssize\systemem \tm + 1 & 
   \syssize\systemem {\tm \mm{\tmtwo}} &:= &\syssize\systemem \tm + \syssize\systemem \tmtwo 
   \end{array} \] 
\paragraph{Memory contexts.}
Memory operators occur at any position of a term, and
their occurrences do not prevent $\beta$-reduction to be fired, so that 
we need \emph{memory contexts} to properly define the notion of evaluation: 
\[ \mctx :: = \Box \mid \mctx\mm{\tm} \] 
%An \emph{$\mem$-abstraction} is a term of the form $\putinctx{\mctx}{\l \var. \tm}$. 

\begin{figure*}
  \centering
  \ovalbox{\small
    $\begin{array}{c}
      \textsc{$\mem$-abstraction} \\[3pt]
      \delia{\infer{\absmem {\l \var. \tm} }{ \phantom{\spneumem{x}} } \quad
      \infer{\absmem {\tm\mm{\tmtwo} }}{\absmem \tm }} \\\\[-3pt]
   \hline\\[-8pt]      
      \textsc{$\mem$-Spine normal forms} \\[3pt]
   \infer{\spneumem{x} }{ \phantom{\spneumem{x}} } \quad
   \infer{\spneumem{\tm \tmtwo}}
         {\spneumem{\tm}} \quad
   \infer{\spneumem{\tm\mm{\tmtwo}}}
         {\spneumem{\tm}} \quad
   \infer{\spnormmem{\tm}}
         {\spneumem{\tm}}\quad
   \infer{\spnormmem{\l \var. \tm}}
         {\spneumem{\tm}} \\\\[-3pt]
   \hline\\[-8pt]
   \textsc{$\mem$-Skeleton normal forms} \\[3pt]
      \infer[]{\skeneumem{\var}}{ \phantom{\skeneumem{\var}} } 
      \sep  
      \infer[]{ \skeneumem{\tm \tmtwo} }
              { \skeneumem{\tm} \quad \skenormmem{\tmtwo}} 
      \sep
      \infer[]{ \skeneumem{\tm \mm{\tmtwo}} }
              { \skeneumem{\tm} \quad \skenormmem{\tmtwo}}
      \\  \\
      \infer[]{ \skenormmem{\tm} }
              { \skeneumem{\tm}  } 
      \sep  
      \infer[]{ \skenormmem{\la\vartwo\tm} }{ \skenormmem{\tm}} 
      \sep 
      \infer[]{ \skenormmem{\tm\mm{\tmtwo}}}
        { \skenormmem{\tm} \quad \skenormmem{\tmtwo} }
      \end{array}      
   $ }
  \caption{Spine  and skeleton neutral and normal forms for $\mem$-terms}
  \label{fig:normalformsmemory}
\end{figure*}


\begin{figure*}
  \centering
  \ovalbox{
    $\begin{array}{c}
      \infer[\toperpmax]
        {\putinctx{\mctx}{\l x. \tm}\tmtwo   \toperp  \putinctx{\mctx}{\tm \isub \var \tmtwo}}
        { \phantom{\var \notin  \ifv{\tm} \mbox{ or } \skenormmem{\tmtwo}}}
   \msep 
 \infer[\topermaxone]
        {\putinctx{\mctx}{\l x. \tm}\tmtwo   \toperp \putinctx{\mctx}{\l x. \tm}\tmthree }
        { \tm \in \specialterms{\var} \msep   \tmtwo \toperp \tmthree}
  \msep           
  \infer[\toperpmappr]
        {\tmthree \tm \toperp \tmthree \tmtwo}
        {\spneumem{\tmthree} \sep  \tm \toperp  \tmtwo}
  \\ \\ 
  \infer[\toperpmappl]
        {\tm \tmthree \toperp  \tmtwo \tmthree}
        {\tm \toperp \tmtwo}
   \msep 
  \infer[\toperpmabs]
        {\la\var \tm \toperp \la\var \tmtwo}
        {\tm \toperp \tmtwo} 
   \msep 
  \infer[\mmemii]
         {\tm \mm{\tmtwo}  \toperp  \tm  \mm{\tmthree}}
         {\tmtwo  \toperp  \tmthree}
  \msep 
   \infer[\mmemi]
        {\tm \mm{\tmthree}  \toperp  \tmtwo \mm{\tmthree}}
        {\tm  \toperp  \tmtwo}
     \end{array} $ 
  }
  \caption{Non-Deterministic Skeleton Evaluation for $\mem$-Terms}
  \label{fig:memory-discipline}
\end{figure*}


\begin{proposition}[Memory \delia{bievaluation systems}]
\label{prop:memory-bievaluation}
  Let $(\system,\detsystem) \in \set{(\toperp,\toperpp)}$.
  Then $(\lterms_{\mem},\toperp, \toperpp, \sysneutralpr \systemem, \sysnormalpr \systemem, \sysabspr \systemem)$ is \delia{a bievaluation system}.
\end{proposition}

\delia{
  \begin{proof} The proof is standard. In rule $\topermaxone$
    of \reffig{memory-discipline}, remark that
  the condition $\tm \in \specialterms{\var}$ implies
  $\tm = \tm'\mm{\var}$ and $\var \notin \fv{\tm'}$, 
  which is essential to obtain the diamond property
  for $\toperp$. %Also, $\numifv{\tm}{\var}=1$ implies   $\numfv{\tm}{\var} = 1$.
  
\end{proof}}
 


%% \begin{lemma}[Properties of Memory  Small-Step Evaluation]
%% \label{l:memory-eval-prop}\hfill
%% \begin{enumerate}
%% \item \label{p:memory-eval-prop-determ} \emph{Diamond}: 
%% if $\tm \toperp \tm_i\ (i=1,2)$, then there is 
%% $\tm_3$ such that  $\tm_i \toperp  \tm_3\ (i=1,2)$.

%% \item \label{p:memory-eval-prop-charac}\emph{Characterization of
%% $\toperp$-normal forms}: $\tm$ is $\toperp$-normal iff $\skenormmem \tm$.
%% Moreover,  $\tm$ is $\toperp$-normal and $\notabsmem \tm$  iff 
%% $\skeneumem\tm$.  
%% \end{enumerate}
%% \end{lemma}


%% \begin{proof} By induction. 
%% \end{proof}


\begin{figure*}
  \centering
  \ovalbox{
\[\begin{array}{c}
  \infer[]
        {\putinctx{\mctx}{\l x. \tm}\tmtwo   \toperpp  
         \putinctx{\mctx}{\tm \isub \var \tmtwo}}
        { \delia{\tm \notin \specialterms{\var}} \mbox{ or } \skenormmem{\tmtwo} }
  \msep 
 \infer[]
        {\putinctx{\mctx}{\l x. \tm}\tmtwo   \toperpp \putinctx{\mctx}{\l x. \tm}\tmthree }
        { \delia{ \tm \in \specialterms{\var}} \msep   \tmtwo \toperpp \tmthree} 
 \msep 
  \infer[]{\la\var \tm \toperpp \la\var \tmtwo}
                    {\tm \toperpp \tmtwo}
  \\ \\
   \infer[]{\tm \tmthree \toperpp  \tmtwo \tmthree}
                     {\notabsmem {\tm} \msep \tm \toperpp \tmtwo } 
  \msep 
                     \infer[]{ \tmthree \tm \toperpp \tmthree \tmtwo}
                      { \skenormmem \tmthree  \msep \tm \toperpp  \tmtwo}
  \msep 
    \infer[]{\tmthree\mm{\tm }  \toperpp  \tmthree \mm{\tmtwo} }
            {    \tm  \toperpp  \tmtwo }
    \msep 
     \infer[]{\tm \mm{\tmthree}  \toperpp  \tmtwo \mm{\tmthree}  }
           { \skenormmem \tmthree \msep   \tm  \toperpp  \tmtwo  
           }
  
\end{array} \]
}
\caption{Deterministic Skeleton Memory Evaluation}
  \label{fig:memory-deterministic}
\end{figure*}

As a consequence,  given $\tm \toperp^k \tmtwo$, where $\skenormmem\tmtwo$, then
there is an evaluation sequence  $\tm \toperpp^k \tmtwo$, with same source and same
target and having same lenght. 

\paragraph{Multi Types.}
Types and multi types are defined exactly as in Sec.~\ref{sec:typing} but
all  multisets are  now \emph{non-empty}. This is because  empty multisets,
used to type erasable subterms, 
have  no sense in non-erasing
evaluation disciplines such as the presented one above. 

\paragraph{Typing System. }
The type system $\systemem$ for $\mperpe$-evaluation is defined
 in Fig.~\ref{fig:type-system-memory}.
\begin{figure}[!h]
  \centering
  \ovalbox{
\begin{tabular}{c}
\mbox{ Typing rules 
$\{ \ax, \many, \funsteps, \funresult, \appsteps, \appresult<\ske>\}$ } \mbox{ plus } \\ \\
$\infer[\mem]{\Deri
            [(\steps + \steps', \result + \result')]
            {\typctx \uplus  \typctxtwo}
            {\tm \mm{\tmtwo}} \typetwo}
            {\Deri[(\steps, \result)] \typctx \tm {\typetwo}
             \quad
             \Deri[(\steps', \result')] {\typctxtwo} \tmtwo {\typethree}}$\\
\end{tabular}
}
\caption{Type System for Memory Skeleton  Evaluation}
\label{fig:type-system-memory}
\end{figure}  
Remark that rule $\many$ cannot derive now a sequent of the form
$\tyjn{(\spine,\result)}{\tm}{\es}{\emm}$ since the empty multi type
is no more in the grammar of types.
\delia{We define the \emph{size} $\syssize\systemem\tderiv$ of a typing derivation $\tderiv$
as the number of rule applications in $\tderiv$,
not counting rules $\{\ax, \many, \mem\}$.
}

\begin{remark} \mbox{}
\begin{enumerate}
\item \emph{Indicies and typing size}: As in the case of 
systems $\spi$ and $\ske$,  if 
$\tderiv$ types $\tm$ with indicies $(\steps, \result)$, 
then $\steps + \result = \syssize\systemem\tderiv$ for the redefined
notion of size given above (rule $\mem$ does not count in the size). 
%% \begin{lemma}[Triples Encode the Size]
%% \label{l:typing-size}
%% Let $\tderiv \exder[\systemem] \Deri[(\steps, \result)]{\typctx}{\tm}{\type}$ be a typing derivation. Then $\syssize\mem\tderiv = \steps + \result $.
%% \end{lemma}
\item \emph{Relevance}: in contrast to the relevance property of systems
$\spi$ and $\ske$, where typed terms may contain untyped subterms,
an easy induction on typing derivations shows here that a variable appears explicitly  in the typing context \emph{if and only if} it occurs \delia{free} in some subterm (they are all typed now). 
%% \begin{lemma}[Relevance]
%% \label{lem:memory-relevance}
%% If $\tderiv \exder[\systemem] \Deri[(\steps, \result)]{\typctx}{\tm}{\type}$, then $\fv{\tm} = \dom{\typctx}$.
%% \end{lemma}
\item \emph{Vacuous abstractions}: 
since multiset types are not empty in system $\systemem$,
it is not possible to abstract a variable $\var$ not explicitly occurring in 
its typing  context
(\ie\ not free in the term). 
Indeed, if $\var \notin \dom{\typctx}$, then
$\typctx(\var)$ is $\emm$, but since 
$\emm \to \sig$ is not a valid type of the system, 
then no valid typing rule can be applied. 
\end{enumerate}

\end{remark}


\delia{\paragraph{Tight derivations.}
As in the case of systems $\spi$ and $\ske$, there is a simple 
description of a class of typing derivations in  system $\systemem$ 
that provide \emph{exact} bounds for memory evaluation $\toperp$. 
However, the new notion of tight derivation in $\systemem$ must
take into account the typing of memory operators, which are also
evaluated to normal form by means of $\toperp$. However, the type
of a memory operator is independent of the type of the term
where this operator occurs (\cf\ rule $\mem$ in \reffig{type-system-memory}). Thus, 
any tight derivation must tighly type all its memory operators. This gives the
following definition:


}

\begin{definition}[Memory tight derivations]
A derivation $\tderiv \exder[\systemem] \Deri[(\steps, \result)]{\typctx}{\tm}{\typetwo}$
  is \emph{memory tight},  written \mprecise,
  if $\tderiv$ is \precise\ and
  every instance of rule 
  $\mem$ in  $\tderiv$ also verifies  $\tightpred\typethree$. 
\end{definition}




\subsection{Tight correctness}
Correctness of tight typings in system $\systemem$ follows \emph{exactly}
the same scheme used for systems $\spi$ and $\ske$: a substitution lemma
(\reflemma{typing-substitution-memory}), a quantitative subject reduction property (\reflemma{subject-perp-reduction})
and the properties of tight typings of $\mem$-normal forms (\refprop{typing-normal-forms}).



\begin{lemma}[Substitution and Typings for $\systemem$]
  \label{l:typing-substitution-memory}
  The following rule is admissible in  systems $\systemem$:
  \[
   \infer[\delia{\subslemma}]{
     \Deri[(\steps + \steps', \result + \result')]
          {\typctx\mplus\typctx'}{\tm\isub\var\tmtwo }{\typetwo}
   }{
     \Deri[(\steps, \result)] {\typctx; \var: {\M}} {\tm}{\typetwo}
     \quad
     \Deri[(\steps', \result')]{\typctx'} {\tmtwo}{{\M}}
   }
  \]
  Moreover if the derivations of the premisses are \mprecise %(resp. semi-communicative),
  then so is the derivation of the conclusion.
\end{lemma}


\begin{lemma}[Quantitative Subject Reduction for $\systemem$]
  \label{l:subject-perp-reduction} % \refpoint{subject-head-reduction-no-hyp}
If $\tderiv \exder[\systemem] \Deri[(\steps, \result)]{\typctx}{\tm}{\type}$,
and $\mprecisepred{\Phi}$, 
and  $\tm \toperp \tmtwo$, then $\steps \geq 2$ and 
    there exists  $\tderivtwo$ such that  $\mprecisepred{\Phi'}$
    $\tderivtwo \exder[\systemem] \Deri[(\steps-2, \result)]\typctx{\tmtwo}\type$.
    \end{lemma}


\delia{\begin{proposition}[Properties of $\mem$-tight typings for normal forms]
\label{prop:typing-normal-forms}
If $\skenormmem\tm$
and  $\tderiv \exder[\systemem] \tyjn{(\steps, \result)} \tm \typctx \type$
is typing  derivation.
\begin{enumerate}
\item \emph{Size bound}: $\syssize\systemem\tm \leq \syssize\systemem\tderiv$.
\item \emph{Tightness}: if $\tderiv$ is \mprecise\ then  $\steps  = 0$
and $\result = \syssize\systemem\tm$. 
\item \emph{Neutrality}:  if $\type=\neutype$ then
$\skeneumem\tmtwo$. 
\end{enumerate}
\end{proposition}
}

As in the previous cases of $\spi$ and $\ske$, \refprop{typing-normal-forms}
relies on the following key lemma:

\begin{lemma}[Tight Spreading on neutral terms]
  \label{l:memory-whn}
  If $\spneumem{\tm}$ and 
  $\tderiv \exder[\systemem]  \Deri[(\steps, \result)] {\typctx}{\tm}{\type}$
  verifies $\tightpred{\typctx}$, then $\tightpred\type$.
\end{lemma}


All the previous steps together provide the tight correctness theorem:


\begin{theorem}[Memory Tight Correctness]
  \label{th:mem-perp-correctness} % \reftm{correctness}
If $\tderiv \exder[\systemem] \Deri[(\steps, \result)] {\typctx}{\tm}{\type}$
  is \mprecise,
  then there exists $\tmtwo$ such that
  $\sysnormal\systemem\tmtwo$,
  $\tm  \Rewn[\steps/2]{\systemem} \tmtwo$ and $\syssize\systemem\tmtwo = \result$.
  Moreover, if $\type=\neutype$
  then $\sysneutral\systemem\tmtwo$.
\end{theorem}


\subsection{Tight Completeness}

\paragraph{Memory Tight Correctness}
Completeness  of tight typings in system $\systemem$ follows \emph{exactly}
the same scheme used for systems $\spi$ and $\ske$: 
normal forms are tightly typable
(\reflemma{}), anti-substitution lemma (\reflemma{anti-substitution-memory}), and 
quantitative subject reduction (\reflemma{}). 




\begin{proposition}[Normal forms are tightly typable]
\label{prop:max-normal-forms-are-tightly-typable} 
 Let $\tm$ be a $\toperp$ normal form. Then 
 \begin{enumerate}  
  \item \label{p:max-normal-forms-are-tightly-typable-precise}
  \emph{\Precise typing of $\toperp$  normal forms}: there exists a \mprecise\ typing $\tderiv$ for $\tm$. 
  \item \label{p:max-normal-forms-are-tightly-typable-neutral}
  \emph{Neutrality}: moreover, if $\skeneumem\tm$  then $\tderiv$ types $\tm$ with $\neutype$;
  \end{enumerate}
\end{proposition}

% !TEX root = main.tex



\begin{lemma}[Anti-Substitution and Typings for $\systemem$]
  \label{l:anti-substitution-memory}
  Let $\tderiv \exder[\systemem]  \tyjn{(\steps, \spine)}{\tm\isub\var\tmtwo } \typctx \type$.
  Then there exists 
  \begin{itemize}
  \item a multiset $\M$;
  \item a typing derivations $\tderiv_{\tm} \exder[\systemem]  \tyjn{(\steps_{\tm}, \spine_{\tm})}{\tm} 
  {\typctx_{\tm};  \var \col \M} \type$ 
  \item a typing derivation $\tderiv_{\tmtwo} \exder[\systemem]  
  \tyjn{(\steps_{\tmtwo}, \spine_\tmtwo)}{\tmtwo } {\typctx_{\tmtwo}} {\M}$
  \end{itemize}
 such that:
\begin{itemize}
\item \emph{Typing Context}: $\typctx = \typctx_{\tm} \mplus  \typctx_{\tmtwo}$;
\item \emph{Indices}: $(\steps, \spine) = (\steps_{\tm} + \steps_\tmtwo, \spine_{\tmtwo} + \spine_\tmtwo)$.
  \end{itemize}
Moreover, if $\tderiv$ is \mprecise\ then so are $\tderiv_{\tm}$ and $\tderiv_{\tmtwo} $. 
\end{lemma}


\begin{proof} 
  By induction on $\tderiv$ and case analysis on $t$. 
\end{proof}


%% \begin{lemma}[Normal Forms Memory]
%%   \label{l:perp-normal-forms} % \reflemmap{head-normal-forms}{precise}
%%  \delia{lemme a revoir}
%%   Let $\tm$ be a normal form with $\fv\tm = \set{\var_1, \ldots, \var_m}$.
%%   Then there exists a unique \precise typing for $t$,
%%   of the form
%%   \[\tderiv \tri \Deri[(0, \msize\tm)] {\var_1:\mtight_1, \ldots, \var_n:\mtight_n} \tm \nf\] 
%%   where $\size{\mneutral_i} = \fvocv \tm {\var_i}$ for $i \in \set{1, \ldots, n}$.
%%   Moreover, if $\headvar{\tm}$, then the type of $\tm$ is $\neutype$.
%%   \sgl{Isn't this a more precise formulation of Proposition~\ref{prop:max-normal-forms-are-tightly-typable}?}

%% \end{lemma}

%% \input{\proofspath/memory-ev-normal-forms-tight}


%% \begin{lemma}[Subject Maximal Expansion]
%% \label{l:subject-expansion}
%% If $\tm \toperpE E \tmtwo$ and
%% $\tderiv \tri \tyjn{(\steps, \result, \garbage)}\tmtwo\typctx\type$
%% then there exists $\tderivtwo$ such that
%% $\tderivtwo \tri \tyjn{(\steps', \result', \garbagetwo')}\tm{\typctx'}{\type'}$
%% with $\stepstwo \geq \steps+2$.
%% \begin{itemize}
%% \item Non-erasing case:
%%   If $E$ is empty then $\tderivtwo$ can be chosen so that
%%   $\typctx'=\typctx$, $\type'=\type$, $\result'=\result$, $\garbage'=\garbage$.
%% \item\Preciseness:
%%   If $\tderiv$ is \precise then $\tderivtwo$ can be chosen so that
%%   $\stepstwo = \steps + 2$.
%% \end{itemize}
%% \end{lemma}

\begin{lemma}[Quantitative Subject Expansion for $\systemem$]
\label{l:perp-subject-expansion}
Let 
$\tderiv \exder[\systemem]  \Deri[(\steps, \result)]\typctx\tmtwo\type$
be a \mprecise\  derivation. 
%% with all the types of $\typctx$ being $\nf$.
%% Assume any of the following hypotheses holds:
%% \begin{itemize}
%% \item $\Neutral\tm$,
%% \item $\tderiv$ is \precise,
%% \end{itemize}
If $\tm \toperp \tmtwo$, then 
exists a \mprecise\  derivation $\tderiv'$ such that
$\tderivtwo \exder[\systemem]  \Deri[(\steps+2, \result)]{\typctx}\tm{\type}$.
\end{lemma}



\begin{theorem}[Memory Completeness]
\label{th:completeness-mem}
  If $\tm \toperp^k \tmtwo$ where  $\memnormal \tmtwo$, 
  there exists a %% unique
  \mprecise derivation  for $t$
  of the form 
  $\tderiv \exder\Deri[(2k, \syssize\systemem\tmtwo)]\typctx\tm\type$.  
\delia{Moreover, if  $\sysneutral\systemem\tmtwo$, then $\type =\neutral$.}
\end{theorem}


==> 2.2-pure.tex <==
\subsection{A direct approach}
\label{s:SNdirect}

\sgl{This section should eventually be erased}


\begin{lemma}[Subject Maximal Reduction -- Non-erasing Case]
  \strut\label{l:subject-perp-reduction} % \refpoint{subject-head-reduction-no-hyp}

  Let $\tingD{\tderiv}{\tyjn{(\steps, \result)}{\tm}\typctx\type}$.

  \begin{enumerate}

  \item \emph{Head Case}: If $\tm \toh \tmtwo$ without erasing the argument,
    then $\steps\geq 2$ and
    there exists $\tderivtwo$ such that
    $\tderivtwo\tri \tyjn{(\steps-2, \result)}{\tmtwo}\typctx\type$
    (and so $\size\tderivtwo < \size\tderiv$).

  \item \emph{Maximal Case}: if $\tm \toperpNE \tmtwo$
    then $\steps\geq 2$ and
    there exists $\tderivtwo$ such that
    $\tderivtwo\tri \tyjn{(\stepstwo, \result)}{\tmtwo}\typctx\type$ with
    \begin{enumerate}
    \item \label{p:subject-head-reduction-no-hyp}
      \emph{No Further Hypotheses}:
      $\stepstwo \leq \steps-2$
      (and so $\size\tderivtwo < \size\tderiv$);
    \item \label{p:subject-head-reduction-precise}
      \emph{\Precise}:
      if $\tderiv$ is \precise,
      then $\stepstwo = \steps - 2$.
    \end{enumerate}
  \end{enumerate}
\end{lemma}


\begin{definition}[Neutral head-normal terms]
  The predicate $\nhnormal \tm$ is defined by the following rules:
  \[\begin{array}{c}

  \infer{\nhnormal \var}{\strut}
  \qquad
  \infer{\nhnormal {\tm \tmtwo}}{\nhnormal \tm \quad \Neutral \tm}

  \end{array}
  \]
\end{definition}


\begin{lemma}[\Preciseness for neutral head normal terms]
  \label{l:perp-whn}
  If $\tderiv \exder \Deri[(\steps, \result)] {\typctx}{\tm}{\type}$,
  $\tightpred \typctx$ and $\nhnormal\tm$, then $\type=\nf$.
\end{lemma}
\begin{proof}
  By induction on $\nhnormal\tm$:
  \begin{itemize}
  \item If $\tm$ is $\var$, then from $\tightpred \typctx$ we get $\type=\neutral$.
  \item If $\tm$ is $\tmtwo\tmthree$,
    then whichever typing rule is used for $\tm$, we have a typing derivation
    $\tderiv' \exder \Deri[(\steps', \result')] {\typctx}{\tmtwo}{\typetwo}$
    and $\nhnormal\tmtwo$, so by \ih we have $\typetwo=\neutral$
    and therefore $\tm$ must be typed by rule $(\appresult)$.
    This in turn forces $\type=\neutral$.
  \end{itemize}
\end{proof}


\begin{theorem}[Correctness]
  \label{tm:perp-correctness} % \reftm{correctness}
  Let $\tderiv \exder \Deri[(\steps, \result)] {\typctx}{\tm}{\type}$.
  \begin{enumerate}
  \item If $\tm$ is $(\la\var\tm_0)\tmtwo\tm_1\ldots\tm_n$ and $\var\not\in\fv{\tm_0}$,
    then there exists a derivation
    $\tderiv'\exder \Deri[(\steps', \result')]
    {\typctx'}{\tm_0\tm_1\ldots\tm_n}{\type}$
    with $\steps'\leq\steps-2$, $\result'\leq\result$, 
    and $\tm\toperpE E^k\tm_0\tm_1\ldots\tm_n$ for some $k\leq (\steps-\steps')/2$.
    Moreover if $\tightpred \typctx$ and $\tderiv$ is \intprecise
    then
    $\tightpred {\typctx'}$,
    $\tderiv'$ is \intprecise,
    $k= (\steps-\steps')/2$,
    and $\Sigma_{\tmthree\in E}\size\tmthree = \result-\result'$.
  \item
    There exist $k\leq \steps/2$, $E$ and a normal form $\tmtwo$ such that
    $\tm\toperpE E^k\tmtwo$ and
    \begin{enumerate}
    \item \emph{Neutrality}: \label{p:correctness-one} % 
      if $\tderiv$ types $\tm$ with $\neutype$ then $\tmtwo$ is neutral.
      
    \item \emph{\Preciseness}: if $\tderiv$ is \precise then 
      \begin{enumerate}
      \item \emph{Steps}: $k=\steps/2$, and 
      \item \emph{Size of the Normal Forms}:
        $\size\tmtwo+\Sigma_{\tmthree\in E}\size\tmthree = \result$.
      \end{enumerate}
    \end{enumerate} 
  \end{enumerate} 
\end{theorem}

\begin{lemma}[Anti-Substitution and Typings]
  \label{l:anti-substitution}
  If
  $\tderiv \tri \tyjn{(\steps, \result)}{\tm\isub\var\tmtwo } \typctx \type$
  and $x\in\fv t$,
  then there exist a non-empty finite set $I$ and typing derivations 
  $\tderivtwo \tri \tyjn{(\stepstwo, \resulttwo)}{\tm} {\typctxtwo, \var \col \mult{\type_i}_{\iI}} \type$ 
  and 
  $(\tderiv_i \tri \tyjn{(\steps_i, \result_i)}{\tmtwo } {\typctxtwo_i} {\type_i})_{\iI}$
  such that:
  \begin{itemize}
  \item \emph{Typing Context}: $\typctx = \typctxtwo +_{\iI} \typctxtwo_i$;

  \item \emph{Triple}:
    $(\steps, \result)
    = (\steps' +_{\iI} \steps_i,
    \result' +_{\iI} \result_i -\size I)$.

  \item \emph{Preservation of \intpreciseness}:
    If $\tderiv$ is \intprecise then $\tderivtwo$ and $\tderiv_i$ are all \intprecise.
  \end{itemize}
\end{lemma}


\begin{theorem}[Normal Forms]
  \label{tm:perp-normal-forms} % \reflemmap{head-normal-forms}{precise}
  Let $\tm$ be a normal form with $\fv\tm = \set{\var_1, \ldots, \var_m}$.
  Then there exists a unique \precise typing for $t$,
  and it is of the form $\tderiv \tri \Deri[(0, \size\tm, 0)] \typctx \tm \nf$.
  Moreover, $\tderiv$ is a type derivation of $\tm$ of minimum size, 
  and $\typctx = {\var_1:\mneutral_1, \ldots, \var_n:\mneutral_n}$
  with $\size{\mneutral_i} = \fvocv \tm {\var_i}$ for $i \in \set{1, \ldots, n}$.
\end{theorem}


\begin{lemma}[Subject Maximal Expansion]
  \label{l:perp-subject-expansion}
  Let $\tm \toperpE E \tmtwo$ and
  $\tderiv \exder \Deri[(\steps, \result)]\typctx\tmtwo\type$
  with $\tightpred \typctx$ and $\tderiv$ is \intprecise.
  Assume any of the following hypotheses holds:
  \begin{itemize}
  \item $\Neutral\tm$,
  \item $\tderiv$ is \precise,
  \item $E$ is empty.
  \end{itemize}
  Then there exists $\tderiv'$ such that
  $\tderivtwo \exder \Deri[(\steps+2, \result+\Sigma_{\tm'\in E}\size{\tm'})]{\typctx'}\tm{\type}$
  with $\tightpred {\typctx'}$ and $\tderiv'$ is \intprecise.
  Moreover if $E$ is empty then $\tderiv'$ can be chosen so that $\typctx'=\typctx$.
\end{lemma}

\begin{theorem}[Completeness]
  If $\tm \toperpE E^k \tmtwo$ with $p$ in normal form,
  there exists a %% unique
  \precise typing for $t$,
  and it is of the form 
  $\tderiv \exder\Deri[(2k, \size\tmtwo+\Sigma_{\tm'\in E}\size{\tm'})]\typctx\tm\nf$.
  %% Moreover, $\tderiv$ is a type derivation of $\tm$ of minimum size.
\end{theorem}


==> xstring.tex <==
%  __________________________________________________
% |                                                  |
% |                                                  |
% |                   xstring v1.7c                  |
% |                                                  |
% |                  13 octobre 2013                 |
% |                                                  |
% |__________________________________________________|
%
% This is xtring.tex
%
% "xstring" package consists of the 7 following files:
%   xstring.tex (this file)
%   xstring.sty
%   README
%   xstring_doc_fr.tex, xstring_doc_fr.pdf (manual in french)
%   xstring_doc_en.tex, xstring_doc_en.pdf (manual in english)
%
% Christian Tellechea 2008-2013
% email : unbonpetit@gmail.com
% -------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
%     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% -------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% -------------------------------------------------------------------
\def\xstringversion     {1.7c}
\def\xstringdate        {2013/10/13}
\def\xstringfrenchdate  {13 octobre 2013}
\def\xstringenglishdate {13 october 2013}
\edef\CurrentAtCatcode  {\the\catcode`\@}
\catcode`\@=11
\newwrite\@xs@message% canal pour les messages
\newcount\integerpart
\newcount\decimalpart% compteurs utilis\'es par xstring

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\immediate\write\m@ne{Package: xstring \xstringdate\space\space v\xstringversion\space\space String manipulations}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@gobble#1{}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
\fi% fin des d\'efinitions LaTeX

\long\def\@xs@ifempty#1{%
	\expandafter\ifx\expandafter\relax\detokenize{#1}\relax
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}
% Ouvre un groupe o\`u les catcodes sont \`a 12 et \`a 10 pour les espaces
% ensuite, appelle \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\@xs@MakeVerb{% lit 1 argument et le transforme en verb
	\begingroup% groupe o\`u les catcodes sont \`a 12 pour la lecture suivante
		\def\do##1{\catcode`##112\relax}%
		\dospecials% on entre dans le mode verb
		\obeyspaces% et on tient compte des espaces
		\@xs@ReadVerb% et on va lire l'argument
}

% D\'efinit \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\setverbdelim#1{% d\'efinit quel est le d\'elimiteur de verb
	\expandafter\@xs@ifempty\expandafter{\@gobble#1}%
		\relax
		{\begingroup
			\newlinechar`\^^J%
			\immediate\write\@xs@message
			{Package xstring Warning: verb delimiter is not a single token on input line \the\inputlineno^^J}%
		\endgroup
		}%
	\def\@xs@ReadVerb##1#1##2#1{% lit ##2 qui est entre les d\'elimiteurs de verb
		\endgroup% on ferme le groupe
		\@xs@afterreadverb{##2}}% on appelle l'ex\'ecution de fin
}

% Assigne l'argument entre d\'elimiteur verb dans la sc #1' +
\def\verbtocs#1{%
	\def\@xs@afterreadverb##1{\def#1{##1}}%
	\@xs@MakeVerb
}

\begingroup
	\catcode\z@3 \def\@xs@twochars{^^00}%
	\catcode\z@7 \xdef\@xs@twochars{\@xs@twochars^^00}%
\endgroup

\edef\@xs@reserved@A{\long\def\noexpand\@xs@AssignResult##1\@xs@twochars}

\@xs@reserved@A#2{\endgroup\expandafter\def\expandafter#2\expandafter{\@gobble#1}}

\def\tokenize#1#2{%
	\begingroup
		\@xs@def\@xs@reserved@A{#2}% on d\'eveloppe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\@xs@twochars#1}% met "^^@^^@#1" \`a la fin du fichier virtuel
		\endlinechar\m@ne
		\expandafter\@xs@AssignResult\scantokens\expandafter{\expandafter\relax\@xs@reserved@A}% on fait l'assignation
}%

% Macro tr\`es simple qui assigne ou affiche le r\'esultat, selon la pr\'esence
% ou non de #2 qui est l'argument optionnel venant en derni\`ere position des macros
\long\def\@xs@ReturnResult#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#2}%
		\@xs@argument@A
		{\let#2\@xs@argument@A}%
}

\def\@xs@ldef{\long\def}

\def\@xs@ledef{\long\edef}

% Pas d'expansion des arguments
\def\normalexpandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter{##1}}}
\let\noexpandarg\normalexpandarg% synonyme

% 1-d\'eveloppement du premier token des arguments
\def\expandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

% D\'eveloppement maximum des arguments
\def\fullexpandarg{%
	\let\@xs@def\@xs@ledef% on d\'efinit\@xs@call avec \edef
	\def\@xs@expand##1{##1}% et on neutralise \@xs@expand
}

\def\saveexpandmode{\let\@xs@saved@def\@xs@defarg\let\@xs@saved@expand\@xs@expand}

\def\restoreexpandmode{\let\@xs@defarg\@xs@saved@def\let\@xs@expand\@xs@saved@expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\@xs@ifbeginwithbrace#1{%
	\csname @%
		\expandafter\@gobble\string{%
		\expandafter\@gobble\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@firstoftwo
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\@gobble\string}%
		\@secondoftwo{first}{second}oftwo%
	\endcsname
}

% Cette macro interne prend la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@returnfirstsyntaxunit#1#2{%
	\def\@xs@groupfound{\expandafter\def\expandafter#2\expandafter{\expandafter{#2}}\@xs@gobbleall}% on met #2 dans des accolades et on finit
	\long\def\@xs@assignfirsttok##1##2\@xs@nil{\let\@xs@toks0\def#2{##1}}%
	\def\@xs@testfirsttok{%
		\let\@xs@next\@xs@assignfirsttok
		\ifx\@xs@toks\bgroup
			\expandafter\@xs@ifbeginwithbrace\expandafter{\@xs@argument}{\def\@xs@next{\afterassignment\@xs@groupfound\def#2}}{}%
		\fi
		\@xs@next}%
	\def\@xs@argument{#1}%
	\edef\@xs@next{\expandafter\@xs@beforespace\detokenize{#1} \@xs@nil}% #1 commence par un espace ?
	\ifx\@xs@next\@empty
		\def\@xs@next{\expandafter\ifx\expandafter\@empty\detokenize\expandafter{\@xs@argument}\@empty\let#2\@empty\else\def#2{ }\let\@xs@toks0\fi}%
	\else
		\def\@xs@next{\expandafter\futurelet\expandafter\@xs@toks\expandafter\@xs@testfirsttok\@xs@argument\@xs@nil}%
	\fi
	\@xs@next
}

% Cette macro interne enl\`eve la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@testsecondtoken#1\@xs@nil{\@xs@ifbeginwithbrace{#1}}

\long\def\@xs@gobblespacebeforebrace#1#{}% supprime tout ce qui est avant la 1ere accolade ouvrante

\long\def\@xs@removefirstsyntaxunit#1#2{%
	\def\@xs@argument{#1}%
	\expandafter\expandafter\expandafter\ifx\expandafter\expandafter\expandafter\@empty\expandafter\@xs@beforespace\detokenize\expandafter{\@xs@argument} \@xs@nil\@empty% #1 commence par un espace ?
		\expandafter\@xs@ifempty\expandafter{\@xs@argument}%
			{\let#2\@empty}
			{\afterassignment\@xs@testsecondtoken% après avoir mangé le 1er token, on va tester si la suite commence par «{»
			\expandafter\let\expandafter\@xs@secontoken\expandafter=\expandafter\@sptoken\@xs@argument\@xs@@nil\@xs@nil% on mange le 1er token et on rajoute \@xs@@nil à la fin pour éviter de perdre les accolades du groupe
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@gobblespacebeforebrace\@xs@argument}}%
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@behindspace\@xs@argument\@xs@nil}}%
			}%
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
		\expandafter\expandafter\expandafter{\expandafter\@gobble\@xs@argument}%
	\fi
}

% Macros \`a arguments d\'elimit\'es pour les macros ci dessus
\long\def\@xs@beforespace#1 #2\@xs@nil{#1}

\long\def\@xs@behindspace#1 #2\@xs@nil{#2}

\long\def\@xs@returnfirstsyntaxunit@ii#1#2\@xs@nil{#1}

\long\def\@xs@gobbleall#1\@xs@nil{}

% Cette macro interne est utilis\'ee dans les macros \'etoil\'ees pour :
% 1) d\'evelopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci \`a l'aide de la macro \@xs@def
% 2) Ensuite, on d\'etokenize ce d\'eveloppement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\@xs@expand@and@detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\@xs@expand#1}% on d\'eveloppe #2 selon le mode de d\'eveloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d\'etokenize et on assigne \`a #1
}

\long\def\@xs@expand@and@assign#1#2{\@xs@def#1{#2}}% on d\'eveloppe #2 selon \fullexpandarg ou \normalexpandarg

\long\def\@xs@edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}

\long\def\@xs@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\def\@xs@argstring{0########1########2########3########4########5########6########7########8########9}

% \@xs@DefArg{3} met dans la sc \@xs@myarg les tokens "####1####2####3"
\def\@xs@DefArg#1{\def\@xs@defarg0##1#1##2\@xs@nil{\def\@xs@myarg{##1#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@DefArg@{3} met dans la sc \@xs@myarg les tokens "[####1]####2####3####4"
\def\@xs@DefArg@#1{\expandafter\@xs@defarg@\expandafter{\number\numexpr#1+1}}

\def\@xs@defarg@#1{\def\@xs@defarg0##11##2#1##3\@xs@nil{\def\@xs@myarg{[##11]##2#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@OneArg{3} met dans la sc \@xs@myarg les tokens "####3"
\def\@xs@OneArg#1{\expandafter\@xs@onearg\expandafter{\number\numexpr#1-1}{#1}}

\def\@xs@onearg#1#2{\def\@xs@defarg##1#1##2#2##3\@xs@nil{\def\@xs@myarg{##2#2}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% #1 : num\'ero du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num\'ero de l'argument devant être d\'etokenis\'e si \'etoile
\def\@xs@BuildLines#1#2#3#4{%
	\let\@xs@newlines\@empty
	\let\@xs@newargs\@empty
	\def\@xs@buildlines##1{%
		\expandafter\@xs@OneArg\expandafter{\number\numexpr##1+#1-1}%
		\edef\@xs@reserved@B{\noexpand\@xs@expand\csname @xs@arg@\romannumeral\numexpr##1\endcsname}%
		\ifnum##1=\@ne% si c'est le premier argument
			\@xs@ifempty{#3}%
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
				\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter[\@xs@reserved@B]}%
				\def\@xs@reserved@B{@xs@def}% ne pas d\'etok\'eniser l'argument optionnel grace au \@xs@def
				}
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
			\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
		\fi
		\edef\@xs@newlines{\unexpanded\expandafter{\@xs@newlines}\expandafter\noexpand\csname\@xs@reserved@B\endcsname\expandafter\noexpand\csname @xs@arg@\romannumeral\numexpr##1\endcsname{\@xs@myarg}}%
		\ifnum##1<#2\relax
			\def\@xs@next{\expandafter\@xs@buildlines\expandafter{\number\numexpr##1+1}}%
			\expandafter\@xs@next
		\fi}%
	\@xs@buildlines\@ne
}

\def\@xs@newmacro{%
	\@ifstar
		{\let\@xs@reserved@D\@empty\@xs@newmacro@}
		{\let\@xs@reserved@D\relax\@xs@newmacro@0}%
}

% #1 : dernier num\'ero de l'argument devant être d\'etokenis\'e
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\@xs@newmacro@#1#2#3#4#5{%
	\edef\@xs@reserved@A{@xs@\expandafter\@gobble\string#2}%
	\edef\@xs@reserved@C{\expandafter\noexpand\csname\@xs@reserved@A @\ifx\@empty#3\@empty @\fi\endcsname}%
	\edef\@xs@reserved@B{%
		\ifx\@empty\@xs@reserved@D
			\def\noexpand#2{\noexpand\@ifstar
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@detokenize\expandafter\noexpand\@xs@reserved@C}%
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
		\fi
		\ifx\@empty#3\@empty
		\else
			\def\expandafter\noexpand\@xs@reserved@C{%
				\noexpand\@testopt{\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname}{\ifx\@xs@def\@xs@ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit :
	% si #3 est vide : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@@}}
	% si #3 existe   : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@}}
	%                  \@xs@NOM@{\@testopt{\@xs@NOM@@}{#3}}}
	\long\@xs@reserved@B
	\ifx\@empty#3\@empty
		\@xs@BuildLines1{#4}{#3}{#1}%
		\@xs@DefArg{#4}%
	\else
		\expandafter\@xs@BuildLines\expandafter1\expandafter{\number\numexpr#4+1}{#3}{#1}%
		\@xs@DefArg@{#4}%
	\fi
	\edef\@xs@reserved@B{\def\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname\@xs@myarg}%
	\edef\@xs@reserved@C{\unexpanded\expandafter{\@xs@newlines}\edef\noexpand\@xs@call}%
	\edef\@xs@reserved@D{%
		\noexpand\noexpand\expandafter\noexpand\csname\@xs@reserved@A\endcsname\unexpanded\expandafter{\@xs@newargs}%
	}%
	\ifnum#5=\@ne\edef\@xs@reserved@D{\noexpand\noexpand\noexpand\@testopt{\unexpanded\expandafter{\@xs@reserved@D}}{}}\fi
	\@xs@edefaddtomacro\@xs@reserved@C{{\unexpanded\expandafter{\@xs@reserved@D}}\noexpand\@xs@call}%
	\@xs@edefaddtomacro\@xs@reserved@B{{\unexpanded\expandafter{\@xs@reserved@C}}}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\@xs@NOM@@[##2]##3##4##5{%
	%          \@xs@def\@xs@arg@i{##2}\@xs@assign\@xs@arg@ii{##3}\@xs@assign\@xs@arg@iii{##4}\@xs@asign\@xs@arg@iv{##5}%
	% si #5=0: \edef\@xs@call{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}%
	% si #5=1: \edef\@xs@call{\noexpand\@testopt{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@i}{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}{}}%
	%          \@xs@call}
	\long\@xs@reserved@B
	\edef\@xs@reserved@B{%
		\def\expandafter\noexpand\csname\@xs@reserved@A\endcsname
			\@xs@myarg\ifnum#5=\@ne[\unexpanded{##}\number\numexpr\ifx\@empty#3\@empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \@xs@NOM[##2]##3##4##5[##6]{#6}
	\long\@xs@reserved@B
}

% macro g\'en\'erique qui lit \@xs@reserved@C us par us
% 3 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atbegingroup      (un groupe vient d'être ouvert)
% \@xs@atnextsyntaxunit  (la future US n'est pas un groupe)
\def\@xs@read@reserved@C{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@read@reserved@C
		\@xs@exploregroups
		\ifx\bgroup\@xs@toks
			\advance\integerpart\@ne
			\begingroup
				\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
				\@xs@manage@groupID
				\let\@xs@nestlevel\@ne
				\integerpart\z@
				\@xs@atbegingroup
		\else
			\global\advance\decimalpart\@ne
			\@xs@atnextsyntaxunit
		\fi
		}%
	\@xs@next
}

% macro g\'en\'erique qui lit \@xs@reserved@D en proc\'edant \`a des tests avec \IfBeginWith
% 2 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atoccurfound      (une occurrence a \'et\'e trouv\'ee)
\def\@xs@read@reserved@D{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}%
		{\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
			{\expandafter\@xs@reserved@D\expandafter}\expandafter{\@xs@reserved@E}%
			{\global\advance\decimalpart\@ne
			\let\@xs@reserved@D\@xs@reserved@A
			\@xs@atoccurfound
			}%
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@A
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
			\let\@xs@next\@xs@read@reserved@D
			\@xs@exploregroups
			\ifx\bgroup\@xs@toks
				\advance\integerpart\@ne
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@D\@xs@reserved@A
					\@xs@manage@groupID
					\let\@xs@reserved@C\@empty
					\let\@xs@nestlevel\@ne
					\integerpart\z@
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro\StrRemoveBraces{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\let\@xs@reserved@B\@empty
	\let\@xs@nestlevel\z@
	\@xs@StrRemoveBraces@i
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#2}%
}

\def\@xs@StrRemoveBraces@i{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@B}%
			\let\@xs@next\@xs@StrRemoveBraces@i
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@StrRemoveBraces@i
		\ifx\bgroup\@xs@toks
			\ifx\@xs@exploregroups\relax% on explore les groupes ?
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
					\let\@xs@nestlevel\@ne
					\integerpart\z@
					\let\@xs@reserved@B\@empty
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\@xs@reserved@A
			\fi
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
		\fi
		}%
	\@xs@next
}

% \@xs@cutafteroccur coupe l'argument #1 apr\`es la #3\`eme occurrence de #2
% \@xs@reserved@C : contient ce qui se trouve avant cette occurrence
% \@xs@reserved@D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \@xs@reserved@E : contient ce qui se trouve apr\`es l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy\'ees sont vides
\long\def\@xs@cutafteroccur#1#2#3{%
	\ifnum#3<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
		}
		{\@xs@cutafteroccur@i{#1}{#2}{#3}}%
}
	
\long\def\@xs@cutafteroccur@i#1#2#3{%
	\def\@xs@reserved@D{#1}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#2}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\ifnum\decimalpart=\numexpr(#3)\relax % occurrence trouv\'ee ?
		\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\@xs@argument@A}%
	\else
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
	\fi
}

\@xs@newmacro*3\IfSubStr{1}{2}{0}{%
	\def\@xs@argument@A{#2}\def\@xs@argument@B{#3}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur
	\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter{\@xs@argument@B}{#1}%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*2\IfBeginWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@secondoftwo
		}
		{\def\@xs@next{%
			\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
				{\expandafter\@xs@argument@A\expandafter}\expandafter
				{\@xs@argument@B}}%
		}%
	\@xs@next
}

\long\def\@xs@IfBeginWith@i#1#2{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@firstoftwo% #2 est vide, tous les tests sont pass\'es avec succ\`es : on renvoie #3
		}
		{\expandafter\@xs@ifempty\expandafter{\@xs@argument@A}%
			{\let\@xs@next\@secondoftwo% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
			\ifx\@xs@reserved@A\@xs@reserved@B% il y a \'egalit\'e...
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A% on enl\`eve les 1ere unit\'es syntaxiques
				\def\@xs@next{% et on recommence avec ces arguments racourcis d'1 unit\'e syntaxique
					\expandafter\expandafter\expandafter\@xs@IfBeginWith@i
					\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}}%
			\else
				\let\@xs@next\@secondoftwo
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro*2\IfEndWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\@xs@ifempty{#2}%
		{\let\@xs@reserved@A\@secondoftwo
		}
		{\expandafter\expandafter\expandafter\@xs@StrCount
			\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter
			{\@xs@argument@B}[\@xs@reserved@A]%
		\ifnum\@xs@reserved@A=\z@
			\let\@xs@reserved@A\@secondoftwo
		\else
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
				{\let\@xs@reserved@A\@firstoftwo}
				{\let\@xs@reserved@A\@secondoftwo}%
		\fi
		}%
	\@xs@reserved@A
}

\@xs@newmacro*4\IfSubStrBefore{1,1}{3}{0}{\@xs@IfSubStrBefore@i[#1]{#2}{#3}{#4}}

\def\@xs@IfSubStrBefore@i[#1,#2]#3#4#5{%
	\def\@xs@reserved@C{#3}%
	\ifx\@xs@exploregroups\relax% si on explore les groupes
		\let\@xs@reserved@B\@empty
		\let\@xs@nestlevel\z@
		\@xs@StrRemoveBraces@i% on retire les accolades
		\let\@xs@reserved@C\@xs@reserved@B
	\fi
	\def\@xs@reserved@A{#5}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#2}%
	\def\@xs@reserved@A{#4}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#1}%
	\global\let\groupID\@empty
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*4\IfSubStrBehind{1,1}{3}{0}{\@xs@IfSubStrBehind@i[#1]{#2}{#3}{#4}}

\long\def\@xs@IfSubStrBehind@i[#1,#2]#3#4#5{\@xs@IfSubStrBefore@i[#2,#1]{#3}{#5}{#4}}

\long\def\@xs@formatnumber#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\@xs@returnfirstsyntaxunit{#1}\@xs@reserved@A
		\def\@xs@reserved@B{+}%
		\ifx\@xs@reserved@A\@xs@reserved@B
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@C
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			 	{\def#2{+0X}}
			 	{\expandafter\def\expandafter#2\expandafter{\expandafter+\expandafter0\@xs@reserved@C}}%
		\else
			\def\@xs@reserved@B{-}%
			\ifx\@xs@reserved@A\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
				\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
					{\def#2{-0X}}%
					{\expandafter\def\expandafter#2\expandafter{\expandafter-\expandafter0\@xs@reserved@A}}%
			\else
				\expandafter\def\expandafter#2\expandafter{\expandafter0\@xs@argument@A}%
			\fi
		\fi
		}%
}

\@xs@newmacro\IfInteger{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\let\@xs@after@intpart\@xs@afterinteger
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\ifnum\decimalpart=\z@
			\let\@xs@next\@firstoftwo% partie décimale constituée de 0 --> seul cas où on renvoie vrai
		\else
			\let\@xs@afterinteger\@xs@after@intpart
			\let\@xs@next\@secondoftwo
		\fi
	\else
		\let\@xs@afterinteger\@xs@after@intpart
		\let\@xs@next\@secondoftwo
	\fi
	\@xs@next
}

\@xs@newmacro\IfDecimal{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}

\long\def\@xs@defafterinteger#1\relax\@xs@nil{\def\@xs@afterinteger{#1}}

\def\@xs@testdot{%
	\let\xs@decsep\@empty
	\@ifnextchar.%
		{\def\xs@decsep{.}\@xs@readdecimalpart}%
		{\@xs@testcomma}%
}

\def\@xs@testcomma{%
	\@ifnextchar,%
		{\def\xs@dessep{,}\@xs@readdecimalpart}%
		{\@xs@endnumber}%
}

\long\def\@xs@readdecimalpart#1#2\@xs@nil{%
	\ifx\@empty#2\@empty
		\def\@xs@reserved@A{0X}%
	\else
		\def\@xs@reserved@A{0#2}%
	\fi
	\afterassignment\@xs@defafterinteger\decimalpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@endnumber\@xs@afterinteger\@xs@nil
}

\long\def\@xs@endnumber#1\@xs@nil{\def\@xs@afterdecimal{#1}}

% test d'\'egalit\'e sur des chaines (et des chaines contenant des nombres)
\long\def\@xs@IfStrEqFalse@i#1#2{\let\@xs@reserved@A\@secondoftwo}
\long\def\@xs@IfStrEqFalse@ii#1#2{% renvoie vrai si les 2 arg sont d\'ecimaux et s'ils sont \'egaux, faux sinon
	\@xs@IfDecimal{#1}%
		{\@xs@IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\@xs@reserved@A\@firstoftwo
			\else
				\let\@xs@reserved@A\@secondoftwo
			\fi% les 2 sont d\'ecimaux : on fait le test
			}%
			{\let\@xs@reserved@A\@secondoftwo}% un seul est d\'ecimal
		}%
		{\let\@xs@reserved@A\@secondoftwo}% #1 n'est pas d\'ecimal
}

\long\def\@xs@TestEqual#1#2{% teste si les 2 arguments sont \'egaux
	\def\@xs@reserved@A{#1}\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\let\@xs@reserved@A\@firstoftwo% \'egalit\'e parfaite des 2 chaines
	\else
		\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}%
	\fi
	\@xs@reserved@A
}

\@xs@newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont \'egales
	\let\@xs@reserved@D\@xs@IfStrEqFalse@i
	\@xs@TestEqual{#1}{#2}%
}

\@xs@newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont \'egaux
	\let\@xs@reserved@D\@xs@IfStrEqFalse@ii
	\@xs@TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfStrEq*}\@xs@IfStrCase}%
		{\def\@xs@reserved@E{\IfStrEq}\@xs@IfStrCase}%
}

\long\def\@xs@IfStrCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\def\IfEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfEq*}\@xs@IfEqCase}%
		{\def\@xs@reserved@E{\IfEq}\@xs@IfEqCase}%
}

\long\def\@xs@IfEqCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\long\def\@xs@IfStringCase#1#2[#3]{%
	\long\def\@xs@testcase##1##2##3\@xs@nil{% lit les 2 premieres unit\'es syntaxiques dans ##1 et ##2. Les autres dans ##3
		\@xs@reserved@E{#1}{##1}%
			{##2}% le test est positif, on ex\'ecute le code correspondant
			{\@xs@ifempty{##3}%
			 	{#3}% s'il n'y a plus de cas, on ex\'ecute le code <autres cas>
				{\@xs@testcase##3\@xs@nil}% sinon, on recommence avec ce qui reste
			 }%
	}%
	\@xs@testcase#2\@xs@nil
}

% Renvoie ce qui est \`a gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBefore{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
}

% Renvoie ce qui est \`a droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBehind{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\@xs@newmacro*4\StrBetween{1,1}{3}{1}{\@xs@StrBetween@i[#1]{#2}{#3}{#4}[#5]}

\long\def\@xs@StrBetween@i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\@xs@cutafteroccur{#3}{#5}{#2}%
		\expandafter\@xs@cutafteroccur\expandafter{\@xs@reserved@C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#6}%
	\global\let\groupID\@empty
}

\def\exploregroups{\let\@xs@exploregroups\relax}

\def\noexploregroups{\def\@xs@exploregroups{\let\@xs@toks0\relax}}

\def\saveexploremode{\let\@xs@saveexploremode\@xs@exploregroups}

\def\restoreexploremode{\let\@xs@exploregroups\@xs@saveexploremode}

% Remplace les #1 premi\`eres occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\@xs@newmacro\StrSubstitute{0}{3}{1}{%
	\def\@xs@reserved@D{#2}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#3}%
	\def\@xs@argument@C{#3}\def\@xs@argument@D{#4}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum#1<\@ne
			\let\@xs@reserved@A\@xs@argument@D
		\else
			\ifnum\decimalpart>#1
				\let\@xs@reserved@A\@xs@argument@C
			\else
				\let\@xs@reserved@A\@xs@argument@D
			\fi
		\fi
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
		\@xs@read@reserved@D
	}%
	\@xs@ifempty{#3}%
		{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#5}%
		}
		{\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#5}%
		}%
}

% Supprime les #1 premi\`eres occurrences de #3 dans #2
\@xs@newmacro\StrDel{0}{2}{1}{\@xs@StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\@xs@exitallgroups{\ifnum\@xs@nestlevel>\z@\endgroup\expandafter\@xs@exitallgroups\fi}

% Compte combien d'unit\'es syntaxiques contient la chaine #1 ?
\@xs@newmacro\StrLen{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\decimalpart\z@
	\let\@xs@nestlevel\z@
	\gdef\groupID{0}%
	\let\@xs@atbegingroup\relax
	\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
	\let\@xs@atnextsyntaxunit\relax
	\@xs@read@reserved@C
	\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n\'ecessaire pour trouver une unit\'e syntaxique derri\`ere
\def\@xs@continuetonext{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel>\z@
			\expandafter\endgroup\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}% on concat\`ene
			\expandafter\expandafter\expandafter\@xs@continuetonext% on recommence
		\fi}
		\relax
}%

\def\@xs@manage@groupID{%
	\begingroup\def\@xs@reserved@A{0}%
	\ifx\@xs@reserved@A\groupID% si on arrive du groupe de niveau 0
		\endgroup
		\xdef\groupID{\number\integerpart}% on met simplement le niveau
	\else
		\endgroup
		\expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\groupID\expandafter\expandafter\expandafter{\expandafter\groupID\expandafter,\number\integerpart}%
	\fi
}

% Cette macro coupe la chaine #1 apr\`es l'unit\'e syntaxique n°#2
\def\StrSplit{%
	\@ifstar
		{\let\@xs@reserved@E\@xs@continuetonext\StrSpl@t}%
		{\let\@xs@reserved@E\relax\StrSpl@t}%
}

\@xs@newmacro\StrSpl@t{}{2}{0}{\@xs@StrSplit@i{#2}{#1}\@xs@StrSplit@ii}

% Cette macro interne coupe la chaine #2 apr\`es l'unit\'e syntaxique n°#1
% Le d\'ebut est assign\'e dans \@xs@reserved@B et la fin dans \@xs@reserved@C
\long\def\@xs@StrSplit@i#1#2{%
	\def\@xs@reserved@D{#1}%
	\def\@xs@reserved@C{#2}%
	\let\@xs@reserved@B\@empty
	\global\let\groupID\@empty
	\ifnum#1>\z@
		\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
			\@xs@read@reserved@C
		}%
		\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
		\def\@xs@atnextsyntaxunit{%
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
			\ifnum\decimalpart=\@xs@reserved@D\relax
				\ifx\@xs@reserved@C\@empty\@xs@reserved@E\fi
				\global\let\@xs@reserved@B\@xs@reserved@B
				\global\let\@xs@reserved@C\@xs@reserved@C
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
}

\def\@xs@StrSplit@ii#1#2{\let#1\@xs@reserved@B\let#2\@xs@reserved@C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\@xs@newmacro*3\StrCut{1}{2}{0}{%
	\@xs@ifempty{#3}%
		{\global\let\groupID\@empty
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		}
		{\ifnum#1<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\@xs@StrCut@ii{#2}{#3}1}
			{\@xs@StrCut@ii{#2}{#3}{#1}}%
		}%
	\@xs@StrCut@iii
}

\long\def\@xs@StrCut@ii#1#2#3{%
	\def\@xs@reserved@D{#1}%
	\let\@xs@reserved@C\@empty
	\def\@xs@reserved@E{#2}%
	\decimalpart\z@\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi
	}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter
	\def
		\expandafter\expandafter\expandafter
	\@xs@reserved@D
		\expandafter\expandafter\expandafter
	{\expandafter\@xs@reserved@C\@xs@argument@A}%
}

\long\def\@xs@StrCut@iii#1#2{\let#1\@xs@reserved@C\let#2\@xs@reserved@E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit\'es syntaxiques aux positions compris !
\@xs@newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\@xs@reserved@E\relax
		\@xs@StrSplit@i{#3}{#1}%
		\edef\@xs@reserved@C{\number\numexpr#2-1}%
		\let\@xs@reserved@E\relax
		\expandafter\expandafter\expandafter\@xs@StrSplit@i\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@B}%
	\expandafter\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
	\global\let\groupID\@empty
}

% supprime #2 unit\'es syntaxiques \`a gauche dans la chaine #1
\@xs@newmacro\StrGobbleLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

% extrait de #1 la chaine \`a gauche de longueur #2
\@xs@newmacro\StrLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% supprime #2 unit\'es syntaxiques \`a droite dans la chaine #1
\@xs@newmacro\StrGobbleRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% renvoie #2 unit\'es syntaxiques \`a la droite de la chaine #1
\@xs@newmacro\StrRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

\@xs@newmacro\StrChar{}{2}{1}{%
	\let\@xs@reserved@B\@empty
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\ifnum#2>\z@
		\def\groupID{0}\let\@xs@nestlevel\z@\integerpart\z@\decimalpart\z@
		\let\@xs@atbegingroup\relax
		\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
		\def\@xs@atnextsyntaxunit{%
			\ifnum\decimalpart=\@xs@reserved@D% la n i\`eme US est atteinte ?
				\global\let\@xs@reserved@B\@xs@reserved@A% on capture l'US en cours qui est celle cherch\'ee
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@B}%
		{\global\let\groupID\@empty}
		\relax
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\@xs@newmacro\StrCount{}{2}{1}{%
	\def\@xs@reserved@D{#1}\def\@xs@reserved@E{#2}\let\@xs@reserved@C\@empty
	\@xs@ifempty{#2}%
		{\@xs@ReturnResult{0}{#3}}
		{\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
			\@xs@read@reserved@D
		}%
		\def\@xs@atoccurfound{\let\@xs@reserved@C\@empty\@xs@read@reserved@D}%
		\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro\StrPosition{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\let\@xs@reserved@E\groupID
	\ifx\@xs@reserved@C\@xs@reserved@D
		\@xs@ReturnResult{0}{#4}%
		\let\@xs@reserved@E\@empty
	\else
		\expandafter\@xs@StrLen\expandafter{\@xs@reserved@C}[\@xs@reserved@C]%
		\expandafter\@xs@ReturnResult\expandafter{\number\numexpr\@xs@reserved@C+1}{#4}%
	\fi
	\global\let\groupID\@xs@reserved@E
}

\def\comparestrict{\let\@xs@comparecoeff\@ne}

\def\comparenormal{\let\@xs@comparecoeff\z@}

\def\savecomparemode{\let\@xs@saved@comparecoeff\@xs@comparecoeff}

\def\restorecomparemode{\let\@xs@comparecoeff\@xs@saved@comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont \'egaux et renvoie la
% position de la premiere unit\'e syntaxiques diff\'erente sinon
\@xs@newmacro*2\StrCompare{}{2}{1}{%
	\def\@xs@reserved@A{#1}%
	\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@B\@xs@reserved@A
		\@xs@ReturnResult{0}{#3}%
	\else
		\def\@xs@next{\@xs@StrCompare@i{#1}{#2}{#3}}%
		\expandafter\@xs@next
	\fi
}

\long\def\@xs@StrCompare@i#1#2#3{%
	\def\@xs@StrCompare@iii##1{%
		\let\@xs@reserved@A\@empty
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@reserved@A{*\@xs@comparecoeff}}%
			{\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
				{\def\@xs@reserved@A{*\@xs@comparecoeff}}
				\relax
			}%
		\def\@xs@next{%
			\expandafter\@xs@ReturnResult\expandafter
			{\number\numexpr##1\@xs@reserved@A\relax}{#3}%
		}%
	}%
	\def\@xs@StrCompare@ii##1{% ##1 est la position
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@B
		\ifx\@xs@reserved@B\@xs@reserved@A
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
				{\@xs@StrCompare@iii{##1}% les 2 unit\'es syntaxiques sont \'egales, on renvoie la position
				}
				{\def\@xs@next{\expandafter\@xs@StrCompare@ii\expandafter{\number\numexpr##1+1}}% les 2 unit\'es syntaxiques sont \'egales et non vides, on recommence
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
				}%
		\else% les 2 unit\'es syntaxiques sont diff\'erentes : on renvoie la position
			\@xs@StrCompare@iii{##1}%
		\fi
		\@xs@next
	}%
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\@xs@StrCompare@ii1%
}

\@xs@newmacro\StrFindGroup{}{2}{1}{%
	\def\@xs@reserved@A{#2}\def\@xs@reserved@B{0}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\def\@xs@next{\@xs@ReturnResult{{#1}}{#3}}%
	\else
		\def\@xs@next{\@xs@StrFindGroup@i{#1}{#2}[#3]}%
	\fi
	\@xs@next
}

\long\def\@xs@StrFindGroup@i#1#2[#3]{%
	\def\@xs@StrFindGroup@ii{%
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@next{\@xs@ReturnResult{}{#3}}% s'il ne reste plus rien, on renvoie vide
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@D
			\ifx\bgroup\@xs@toks% si la 1\`ere unit\'e syntaxique est un groupe explicite
				\advance\decimalpart\@ne% on augmente le compteur
				\ifnum\decimalpart=\@xs@reserved@A% on est au groupe cherch\'e lors de la profondeur courante ?
					\ifx\@empty\@xs@reserved@B% on est \`a la profondeur maximale ?
						\def\@xs@next{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#3}}% on renvoie ce groupe
					\else% sinon
						\expandafter\def\expandafter\@xs@next\expandafter{\expandafter\@xs@StrFindGroup@i\@xs@reserved@D}% on recommence avec ce groupe
						\expandafter\@xs@addtomacro\expandafter\@xs@next\expandafter{\expandafter{\@xs@reserved@B}[#3]}% et les profondeurs de recherche restantes
					\fi
				\else
					\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
					\let\@xs@next\@xs@StrFindGroup@ii
				\fi
			\else
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\let\@xs@next\@xs@StrFindGroup@ii
			\fi
			}%
		\@xs@next
	}%
	\@xs@extractgroupnumber{#2}\@xs@reserved@A\@xs@reserved@B
	\decimalpart\z@
	\ifnum\@xs@reserved@A>\z@\def\@xs@reserved@C{#1}\else\let\@xs@reserved@C\@empty\fi
	\@xs@StrFindGroup@ii
}

\def\@xs@extractgroupnumber#1#2#3{%
	\def\@xs@extractgroupnumber@i##1,##2\@xs@nil{\def#2{##1}\def#3{##2}}%
	\@xs@extractgroupnumber@i#1,\@xs@nil
	\ifx\@empty#3\else\@xs@extractgroupnumber@i#1\@xs@nil\fi
}

\def\expandingroups{\let\@xs@expandingroups\exploregroups}

\def\noexpandingroups{\let\@xs@expandingroups\noexploregroups}

\def\StrExpand{\@testopt{\@xs@StrExpand}{1}}
\long\def\@xs@StrExpand[#1]#2#3{%
	\begingroup
		\@xs@expandingroups
		\ifnum#1>\z@
			\integerpart#1\relax
			\decimalpart\z@
			\gdef\groupID{0}%
			\let\@xs@nestlevel\z@
			\def\@xs@atendofgroup{%
				\expandafter\endgroup
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
				\@xs@read@reserved@C
			}%
			\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
			\def\@xs@atnextsyntaxunit{%
				\expandafter\expandafter\expandafter\@xs@addtomacro
				\expandafter\expandafter\expandafter\@xs@reserved@B
				\expandafter\expandafter\expandafter{\@xs@reserved@A}%
			}%
			\def\@xs@reserved@C{#2}%
			\@xs@StrExpand@i{#1}% Appel de la macro r\'ecursive
		\else
			\def\@xs@reserved@B{#2}%
		\fi
		\global\let\@xs@reserved@B\@xs@reserved@B
	\endgroup
	\let#3\@xs@reserved@B
	\global\let\groupID\@empty
}

\long\def\@xs@StrExpand@i#1{%
	\ifnum#1>\z@
		\let\@xs@reserved@B\@empty
		\@xs@read@reserved@C
		\let\@xs@reserved@C\@xs@reserved@B
		\def\@xs@reserved@A{\expandafter\@xs@StrExpand@i\expandafter{\number\numexpr#1-1}}%
	\else
		\let\@xs@reserved@A\relax
	\fi
	\@xs@reserved@A
}

\def\scancs{\@testopt{\@xs@scancs}{1}}
\long\def\@xs@scancs[#1]#2#3{%
	\@xs@StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

% Restaure le code de @
\catcode`\@=\CurrentAtCatcode\relax

% D\'efinit le d\'elimiteur verb
% d\'efinit les diff\'erents modes et les m\'emorise
\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput
%
% Historique
%------------------------------------------------------------------------------
%% v1.0    4/7/2008 : - Package achev\'e.
%          7/7/2008 : - Package publi\'e sur CTAN.
%------------------------------------------------------------------------------
% v1.1    15/8/2008
%   - Le package ne n\'ecessite plus LaTeX et est d\'esormais utilisable sous
%     Plain eTeX.
%   - Ajout des macros \IfInteger et \IfDecimal.
%     Pour cette derni\`ere, la partie enti\`ere et la partie d\'ecimale sont
%     r\'ecup\'erables dans les compteurs \integerpart et \decimalpart. Ce
%     qu'il reste apr\`es qu'un caract\`ere non attendu soit rencontr\'e est
%     dispo dans \@xs@remainafterdecimal
%   - Correction d'un bug dans \tokenize :
%        suppression de l'expansion avec \normalexpandarg pour \'eviter le bug
%        avec les lettres accentu\'ees dans l'exemple : \tokenize\aa{\'e\`u}
%   - Am\'elioration du code de la plupart des macros.
%   - \'Ecriture d'une routine \@xs@newmacro d\'efinissant les  macros.
%   - Suppression de tous les compteurs grace \`a \numexpr.
%   - Nouvelles fonctionnalit\'es internes dans :
%      \IfSubStr
%        ajout des chaines se trouvant avant et apr\`es l'occurrence test\'ee
%        dans les sc \@xs@behind@IfSubStr et \@xs@before@IfSubStr
%      \StrCount
%        a) ajout de ce qui se trouve apr\`es la derni\`ere occurrence dans la
%           sc \@xs@StrCount@afterlastocccur
%        b) la macro ne d\'epend plus d'aucune autre
%------------------------------------------------------------------------------
% v1.2    23/8/2008
%   - Am\'elioration du code de \StrMid \StrGobbleLeft, \StrLeft,
%     \StrGobbleRight et \StrRight \`a l'aide de la nouvelle macro
%     \@xs@StrSplit@i
%   - Nouveau test \IfStrEq qui compare 2 chaines
%   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
%     contiennent un nombre)
%   - Correction d'un bug dans \@xs@formatnumber. La macro n'envisageait pas le
%     cas o\`u son argument \'etait vide ce qui faiasait planter
%     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
%------------------------------------------------------------------------------
% v1.3    21/9/2008
%  - Am\'elioration du code, mise en place de r\'ecursivit\'es terminales dans
%    toutes les macros r\'ecursives, simplification de \@xs@TestEqual en
%    utilisant \ifx
%  - Nouvelles macros \IfStrEqCase et \IfEqCase
%      Teste si une chaîne est \'egale \`a plusieurs cha\^ines donn\'ee et
%      ex\'ecute un code sp\'ecifique
%  - Cr\'eation de la macro publique \StrSplit
%      Coupe la chaine en 2 \`a une position donn\'ee
%  - Nouvelle macro \StrCompare
%      Compare 2 chaînes et renvoie la position du 1er caract\`ere diff\'erent.
%      Renvoie 0 si elles sont \'egales.
%------------------------------------------------------------------------------
% v1.3a   29/9/2008
%  - Correction d'un bug : \expandafter#1
%    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
%    nombre > 9 !
%  - R\'e \'ecriture de \@xs@returnfirstsyntaxunit et \@gobble qui
%    deviennent purement d\'eveloppables.
%  - R\'e \'ecriture de \StrLen
%  - Nouvelle macro interne \@xs@cutafteroccur
%      Coupe la chaine apr\`es la ni\`eme occurrence d'une sous chaine.
%  - Code am\'elior\'e de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
%    \StrGobbleRight grace \`a \@xs@cutafteroccur
%------------------------------------------------------------------------------
% v1.4   4/11/2008
%  - xstring traite ses arguments par unit\'e syntaxique, et donc toutes les
%    macros internes ont \'et\'e r\'e-\'ecrites \`a cette fin.
%  - Le manuel a \'et\'e r\'e-\'ecrit, rendu plus clair et mieux structur\'e.
%  - Nouvelle fonctionnalit\'e : \expandarg
%      le 1er lex\`eme de chaque argument est 1-d\'evelopp\'e avant que la
%      macro ne soit appel\'ee. Si un argument comporte plus qu'1 lex\`eme,
%      il faut passer par \scancs*[1] pour 1-d\'evelopper toutes les unit\'es
%      syntaxiques.
%  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
%    d\'efaut dans \StrSubstitute et \StrDel
%  - Coh\'erence dans les nom des s\'equences de contr\^oles temporaires qui
%    sont d\'esormais : \@xs@reserved@A \`a \@xs@reserved@E
%------------------------------------------------------------------------------
% v1.4a  12/11/2008
%  - Correction d'un bug dans \@xs@StrSplit dans le cas o\`u l'argument
%     num\'erique est <1 : la 1ere coupure doit être vide et le seconde doit
%     être \'egale \`a l'argument.
%------------------------------------------------------------------------------
% v1.4b  16/11/2008
%  - Correction de 2 bugs dans \@xs@returnfirstsyntaxunit
%------------------------------------------------------------------------------
% v1.5   31/12/2008
%  - Nouvelles fonctionnalit\'es dans la recherche de groupes par un
%    identificateur caract\'erisant leur imbrication. Impl\'ementation de :
%      1) \StrFindGroup
%      2) \groupID
%  - Ajout des nouvelles macros g\'en\'eriques \@xs@read@reserved@C et
%    \@xs@read@reserved@D
%  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
%    que \truc contenait «a{a}».
%  - Correction d'un bug dans \@xs@newmacro : l'argument optionnel \'etait
%    d\'etok\'enis\'e \`a tort dans les macros \'etoil\'ees.
%  - Dans \@xs@newmacro, on doit choisir le num\'ero du dernier argument devant
%    être d\'etok\'enis\'e dans le cas d'une macro \'etoil\'ee (sachant que
%     l'argument optionnel ne l'est jamais)
%------------------------------------------------------------------------------
% v1.5a  09/2/2009
%  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
%    indépendante du mode d'exploration et dispose de ses propres commandes
%    d'exploration : \expandingroups et \noexpandingroups
%  - R\'e-\'ecriture de \scancs, qui devient triviale puisque d\'ependant de
%    \StrExpand. Il n'y a plus de version \'étoil\'ee et d\'esormais, \scancs
%    est sensible au mode d'exploration.
%  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
%  - Correction de bugs : mettre \let\@xs@reserved@E\relax avant d'appeler
%    \@xs@StrSplit@i
%  - Suppression des messages d'erreur, de warning et d'info. xstring devient
%    donc silencieux ;)
%  - Passage de 3 \'a 2 compteurs
%  - Le manuel est d\'esormais plus color\'e, en esp\'erant qu'il sera un peu
%    plus agr\'eable \`a lire !
%------------------------------------------------------------------------------
% v1.5b  13/3/2009
%  - Modification d'un grand nombre de macros de telle sorte que vraiment
%    n'importe quel code peut d\'esormais \^etre plac\'e dans les arguments des
%    macros (comme par exemple des \if, \ifx ou autre, m\^eme sans leur \fi, ce
%    qui n'\'etait pas possible jusqu'alors)
%------------------------------------------------------------------------------
% v1.5c  05/6/2009
%  - Correction d'un bug dans \IfBeginWith : il faut appeler
%    \@xs@returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
%    non pas l'inverse pour que \@xs@toks reflète ce qui se trouve dans #1
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit au cas où #1 commence
%    par un espace : mettre \@xs@toks à 0
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit :
%    \@xs@returnfirstsyntaxunit{{}}\truc
%    faisait que \truc se développait en un espace.
%  - Correction d'un bug dans \@xs@removefirstsyntaxunit où le cas
%    \@xs@removefirstsyntaxunit{ {b}}\truc
%    donnait \truc se développant en «b» au lieu de «{b}».
%------------------------------------------------------------------------------
% v1.5d  28/3/2010
%  - Correction d'un bug dans \IfInteger : \@xs@afterinteger ne donnait pas le
%    bon r\'esultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
%  - \xs@formatnumber ne detokenize plus ses arguments (que m'est-il pass\'e
%    par la t\^ete pour que je code un truc comme ca ?), et donc
%    \@xs@afterinteger et \@xs@afterdecimal ont des tokens ayant le bon
%    catcode
%------------------------------------------------------------------------------
% v1.6  24/10/2012
%  - Correction d'un bug dans \@xs@cutafteroccur au cas o\`u #3<1
%  - \IfDecimal ne \detokenize plus l'argument.
%  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
%    \'etait entre accolades
%  - Nouvelle macro \StrCut
%  - \@xs@cutafteroccur@i ne produit plus d'espace indésirable si #3 était
%    évalué par \numexpr
%------------------------------------------------------------------------------
% v1.7  13/1/2013
%  - Correction d'un manque de rigueur dans les assignations concernant
%    \groupID : elles sont toutes globales d\'esormais
%  - Les macros de xstring sont \long
%------------------------------------------------------------------------------
% v1.7a 28/2/2013
%  - Correction d'un espace parasite dans \@xs@removefirstsyntaxunit
%------------------------------------------------------------------------------
% v1.7b 29/7/2013
%  - La date contenue dans \xstringdate est désormais conforme
%------------------------------------------------------------------------------
% v1.7c 13/10/2013 
%  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
